Cooperation in Carrier Sense Based Wireless Ad Hoc Networks - Part I: Reactive Schemes

Cooperative techniques have been shown to significantly improve the performance of wireless systems. Despite being a mature technology in single communication link scenarios, their implementation in wider, and practical, networks poses several challenges which have not been fully identified and understood so far. In this two-part paper, the implementation of cooperative communications in non-centralized ad hoc networks with sensing-based channel access is extensively discussed. Both analysis and simulation are employed to provide a clear understanding of the mutual influence between the link layer contention mechanism and collaborative protocols. Part I of this work focuses on reactive cooperation, in which relaying is triggered by packet delivery failure events, while Part II addresses proactive approaches, preemptively initiated by the source based on channel state information. Results show that sensing-based channel access significantly hampers the effectiveness of cooperation by biasing the spatial distribution of available relays, and by inducing a level of spatial and temporal correlation of the interference that diminishes the diversity improvement on which cooperative gains are founded. Moreover, the efficiency reduction entailed by several practical protocol issues related to carrier sense multiple access which are typically neglected in the literature is thoroughly investigated.

==> csma.tex <==
\section{Carrier Sense Based Multiple Access} \label{sec:csma}

Carrier sense is a fundamental networking mechanism, widely implemented in present day ad hoc networks to control multiple access.\footnote{Throughout this paper we focus on plain carrier sense multiple access (CSMA), epitomized by the IEEE 802.11 DCF without channel negotiation \cite{802.11}, while an investigation including collision avoidance is left as part of future work.} According to CSMA, a terminal that has data to send picks a backoff interval whose duration $n$, in slots, is uniformly drawn in $[0,2^{\textrm{CW}-1}]$, where $\textrm{CW} = \textrm{CW}_{start} + i$, CW$_{start}$ is a system parameter to handle congestion, $i = 0, \ldots, \textrm{SRL}-1$, and SRL is the Short Retry Limit, i.e., the maximum number of transmission attempts performed at the MAC layer before dropping a packet. During this interval, the node senses the aggregate power level on the channel. If the value exceeds the carrier sense threshold, the terminal stops the countdown and freezes the backoff until the medium is sensed idle again for at least a Distributed coordination function InterFrame Space (DIFS) period. On the other hand, once the backoff expires the node transmits its packet. If the destination succesfully decodes the payload, an acknowledgement (ACK) is sent to the source and the communication comes to an end.  Conversely, if the reception fails, no feedback is sent; the source increases its CW counter, and further attempts are performed after newly drawn random backoffs until either the packet is successful or the SRL is reached. 

The simple sensing mechanism implemented  by CSMA allows nodes to acquire information on their neighbors' activity, and is intended both to protect ongoing communications from interference, and to block terminals whose transmissions would  fail with high probability. However, channel impairments such as noise, fading and shadowing as well as the well known hidden and exposed terminal problems~\cite{Tobagi75} may limit the effectiveness of this scheme. Nevertheless, since carrier sense based medium access strategies are widely implemented, they represent a significant  and insightful test environment for cooperative protocols.
